Performance Evaluation of Action Recognition Models on Low Quality Videos

In the design of action recognition models, the quality of videos is an important issue; however, the trade-off between the quality and performance is often ignored. In general, action recognition models are trained on high-quality videos, hence it is not known how the model performance degrades when tested on low-quality videos, and how much the quality of training videos affects the performance. The issue of video quality is important, however, it has not been studied so far. The goal of this study is to show the trade-off between the performance and the quality of training and test videos by quantitative performance evaluation of several action recognition models for transcoded videos in different qualities. First, we show how the video quality affects the performance of pre-trained models. We transcode the original validation videos of Kinetics400 by changing quality control parameters of JPEG (compression strength) and H.264/AVC (CRF). Then we use the transcoded videos to validate the pre-trained models. Second, we show how the models perform when trained on transcoded videos. We transcode the original training videos of Kinetics400 by changing the quality parameters of JPEG and H.264/AVC. Then we train the models on the transcoded training videos and validate them with the original and transcoded validation videos. Experimental results with JPEG transcoding show that there is no severe performance degradation (up to -1.5%) for compression strength smaller than 70 where no quality degradation is visually observed, and for larger than 80 the performance degrades linearly with respect to the quality index. Experiments with H.264/AVC transcoding show that there is no significant performance loss (up to -1%) with CRF30 while the total size of video files is reduced to 30%.

==> fig/acc_ffmpeg_slowfastr101.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.45}
    \def\myimgsclae{0.45}
    \begin{tabular}{cc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slowfast_r101/val_top1acc_0_50_in_original.pdf}
            % \label{fig:slowfast_r101_top1_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slowfast_r101/val_top1acc_bitrate_in_original.pdf}
            % \label{fig:slowfast_r101_top1_bitrate}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slowfast_r101/val_top5acc_0_50_in_original.pdf}
            \subcaption{}
            % \label{fig:slowfast_r101_top5_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slowfast_r101/val_top5acc_bitrate_in_original.pdf}
            \subcaption{}
            % \label{fig:slowfast_r101_top5_bitrate}
        \end{minipage} 
    \end{tabular}
    \caption{
    Recognition rate for video clips transcoded in h.264/AVC with degraded quality.
    The dataset is Kinetics400 and the model is slowfast\_r101.
    Top: top1. Bottom: top5.
    The horizontal axes are (a) the quality parameter CRF and (b) the bit rate, respectively.
    }
    \label{fig:acc_ffmpeg_slowfastr101}
\end{figure*}




==> fig/acc_ffmpeg_slowr50.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.45}
    \def\myimgsclae{0.45}
    \begin{tabular}{cc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slow_r50/val_top1acc_0_50_in_original.pdf}
            % \label{fig:slow_r50_top1_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slow_r50/val_top1acc_bitrate_in_original.pdf}
            % \label{fig:slow_r50_top1_bitrate}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slow_r50/val_top5acc_0_50_in_original.pdf}
            \subcaption{}
            % \label{fig:slow_r50_top5_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/slow_r50/val_top5acc_bitrate_in_original.pdf}
            \subcaption{}
            % \label{fig:slow_r50_top5_bitrate}
        \end{minipage} 
    \end{tabular}
    \caption{
    Recognition rate for video clips transcoded in h.264/AVC with degraded quality.
    The dataset is Kinetics400 and the model is slow\_r50 (ResNet).
    Top: top1. Bottom: top5.
    The horizontal axes are (a) the quality parameter CRF and (b) the bit rate, respectively.
    }
    \label{fig:acc_ffmpeg_slowr50}
\end{figure*}

==> fig/acc_ffmpeg_x3dm.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.45}
    \def\myimgsclae{0.45}
    \begin{tabular}{cc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/x3d_m/val_top1acc_0_50_in_original.pdf}
            % \label{fig:x3d_m_top1_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/x3d_m/val_top1acc_bitrate_in_original.pdf}
            % \label{fig:x3d_m_top1_bitrate}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/x3d_m/val_top5acc_0_50_in_original.pdf}
            \subcaption{}
            % \label{fig:x3d_m_top5_crf}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/acc_ffmpeg/x3d_m/val_top5acc_bitrate_in_original.pdf}
            \subcaption{}
            % \label{fig:x3d_m_top5_bitrate}
        \end{minipage} 
    \end{tabular}
    \caption{Recognition rate for video clips transcoded in h.264/AVC with degraded quality.
    The dataset is Kinetics400 and the model is X3D-M.
    Top: top1. Bottom: top5.
    The horizontal axes are (a) the quality parameter CRF and (b) the bit rate, respectively.}
    \label{fig:acc_ffmpeg_x3dm}
\end{figure*}

==> fig/bitrate.tex <==
\begin{figure*}[tp]
    \centering
    \def\myimgwidth{0.15}
    \def\myimgsclae{0.14}
    \begin{tabular}{p{1.5cm}ccccc}
     & 
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/original_bit_rate.pdf}
            \subcaption{original}
            \label{fig:bitrate_original}
        \end{minipage} \\
    \end{tabular}
    \begin{tabular}{p{1.5cm}|ccccc}
        \diagbox[height=2\line, width=1.9cm]{CRF}{GOP} &  1 & 2 & 5 & 10 & 12 \\ \hline 
        \multicolumn{1}{c|}{0} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf0.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf0.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf0.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf0.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf0.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf0}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{10} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf10.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf10.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf10.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf10.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf10.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf10}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{20} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf20.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf20.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf20.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf20.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf20.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf20}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{30} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf30.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf30.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf30.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf30.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf30.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf30}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{40} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf40.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf40.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf40.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf40.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf40.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf40}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{50} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/1/bit_rate_gop1crf50.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop1crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/2/bit_rate_gop2crf50.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop2crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/5/bit_rate_gop5crf50.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop5crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/10/bit_rate_gop10crf50.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop10crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/bitrate/gop/12/bit_rate_gop12crf50.pdf}
            % \subcaption{original}
            \label{fig:bitrate_gop12crf50}
        \end{minipage} \\
        
    \end{tabular}
    \caption{Histogram of the average bit rate after transcoding in h.264/AVC.
    The horizontal axis represents the bit rate (b/s, logarithmic) and the vertical axis represents the frequency.
    The data used are 19880 videos for Kinetics400 verification.
    (a) is the bit rate of the original video.
    The table shows the bitrates of the compressed video with different GOP and CRF.
    }
    \label{fig:bitrate}
\end{figure*}



==> fig/compare_images_80_100.tex <==
\begin{figure*}[tp]
    \centering
    \def\myimgwidth{0.175}
    \def\myimgsclae{0.37}
    \begin{tabular}{ccccc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/original_frame_0.jpg}
            \subcaption{original}
            \label{fig:80_100_original}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_80.jpg}
            \subcaption{80}
            \label{fig:80_100_80}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_81.jpg}
            \subcaption{81}
            \label{fig:80_100_81}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_82.jpg}
            \subcaption{82}
            \label{fig:80_100_82}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_83.jpg}
            \subcaption{83}
            \label{fig:80_100_83}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_84.jpg}
            \subcaption{84}
            \label{fig:80_100_84}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_85.jpg}
            \subcaption{85}
            \label{fig:80_100_85}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_86.jpg}
            \subcaption{86}
            \label{fig:80_100_86}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_87.jpg}
            \subcaption{87}
            \label{fig:80_100_87}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_88.jpg}
            \subcaption{88}
            \label{fig:80_100_88}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_89.jpg}
            \subcaption{89}
            \label{fig:80_100_89}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_90.jpg}
            \subcaption{90}
            \label{fig:80_100_90}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_91.jpg}
            \subcaption{91}
            \label{fig:80_100_91}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_92.jpg}
            \subcaption{92}
            \label{fig:80_100_92}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_93.jpg}
            \subcaption{93}
            \label{fig:80_100_93}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_94.jpg}
            \subcaption{94}
            \label{fig:80_100_94}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_95.jpg}
            \subcaption{95}
            \label{fig:80_100_95}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_96.jpg}
            \subcaption{96}
            \label{fig:80_100_96}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_97.jpg}
            \subcaption{97}
            \label{fig:80_100_97}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_98.jpg}
            \subcaption{98}
            \label{fig:80_100_98}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_99.jpg}
            \subcaption{99}
            \label{fig:80_100_99}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/images_80_100/compression_rate_100.jpg}
            \subcaption{100}
            \label{fig:80_100_100}
        \end{minipage} 
    \end{tabular}
    
    
    \caption{Variation of image quality with JPEG transcoding
    (compression strength from 80 to 100).}
    \label{fig:compare_images_80_100}


\end{figure*}


==> fig/ffmpeg_kinetics_train.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.32}
    \def\myimgsclae{0.3}
    \begin{tabular}{ccc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/val_acc_top1.pdf}
            \subcaption{}
            \label{fig:x3dm_kinetics_train_val_acc1}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/slow_r50/kinetics400_train/val_acc_top1.pdf}
            \subcaption{}
            \label{fig:slowr50_kinetics_train_val_acc1}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/slowfast_r101/kinetics400_train/val_acc_top1.pdf}
            \subcaption{}
            \label{fig:slowrfastr101_kinetics_train_val_acc1}
        \end{minipage} \\
        
    \end{tabular}
    \caption{Training results using the original video and the video transcoded in h.264/AVC.
    During training, 240194 original videos from the Kinetics400 training set and videos fixed at GOP length 12 and compressed with CRFs of 20, 30, and 40 were used, and during verification, 19880 videos from the verification set of all original videos were used.
    The horizontal axis is the number of epochs and the vertical axis is the recognition rate (top1).
    The models are (a) X3D-M, (b) Slow-R50, and (c) SlowFast-R101.
    }
    \label{fig:ffmpeg_kinetics_train}
\end{figure*}

==> fig/ffmpeg_kinetics_train_x3dm.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.45}
    \def\myimgsclae{0.45}
    \begin{tabular}{cc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/train_loss.pdf}
            \label{fig:x3dm_kinetics_train_train_loss}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/val_loss.pdf}
            \label{fig:x3dm_kinetics_train_val_loss}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/train_acc_top1.pdf}
            \label{fig:x3dm_kinetics_train_train_acc1}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/val_acc_top1.pdf}
            \label{fig:x3dm_kinetics_train_val_acc1}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/train_acc_top5.pdf}
            \subcaption{}
            \label{fig:x3dm_kinetics_train_train_acc5}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/acc_ffmpeg/x3d_m/kinetics400_train/val_acc_top5.pdf}
            \subcaption{}
            \label{fig:x3dm_kinetics_train_val_acc5}
        \end{minipage} \\
        
    \end{tabular}
    \caption{Training results using the original video and the video transcoded in h.264/AVC.
    During training, 240194 original videos from the Kinetics400 training set and videos fixed at GOP length 12 and compressed with CRFs of 20, 30, and 40 were used, and during verification, 19880 videos from the verification set of all original videos were used.
    The number of epochs is 5.5.
    (a) train．(b) val．
    The horizontal axis represents the number of epochs, and the vertical axis represents loss, recognition rate (top1), and recognition rate (top5), starting from the top row.}
    \label{fig:ffmpeg_kinetics_train_x3dm}
\end{figure*}

==> fig/filesize.tex <==
\begin{figure*}[tp]
    \centering
    \def\myimgwidth{0.15}
    \def\myimgsclae{0.14}
    \begin{tabular}{p{1.5cm}ccccc}
     & 
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/original_filesize.pdf}
            \subcaption{original}
            \label{fig:filesize_original}
        \end{minipage} \\
    \end{tabular}
    \begin{tabular}{p{1.5cm}|ccccc}
        \diagbox[height=2\line, width=1.9cm]{CRF}{GOP} &  1 & 2 & 5 & 10 & 12 \\ \hline 
        \multicolumn{1}{c|}{0} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf0.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf0.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf0.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf0.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf0}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf0.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf0}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{10} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf10.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf10.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf10.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf10.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf10}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf10.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf10}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{20} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf20.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf20.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf20.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf20.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf20}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf20.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf20}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{30} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf30.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf30.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf30.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf30.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf30}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf30.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf30}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{40} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf40.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf40.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf40.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf40.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf40}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf40.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf40}
        \end{minipage} \\
        
        \multicolumn{1}{c|}{50} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/1/filesize_gop1crf50.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop1crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/2/filesize_gop2crf50.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop2crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/5/filesize_gop5crf50.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop5crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/10/filesize_gop10crf50.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop10crf50}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[keepaspectratio, scale=\myimgsclae]{images/stream_info_crf_g/filesize/gop/12/filesize_gop12crf50.pdf}
            % \subcaption{original}
            \label{fig:filesize_gop12crf50}
        \end{minipage} \\
    \end{tabular}

    \caption{Histogram of total file size after transcoding in h.264/AVC.
    The horizontal axis shows the file size (in bytes, logarithm), and the vertical axis shows the frequency. The data are 19880 Kinetics400 validation videos.
    (a) is the file size of the original video.
    The table shows the file size of the compressed video with different GOP and CRF.
    }
    \label{fig:filesize}

\end{figure*}



==> fig/jpeg_quality_evaluate.tex <==
\begin{figure*}[t]
    \centering
    \def\myimgwidth{0.22}
    \def\myimgsclae{0.215}
    \begin{tabular}{cccc}
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/0_100/mae_0_100.pdf}
            % \subcaption{ResNet}
            \label{fig:mae_0_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/0_100/rmse_0_100.pdf}
            % \subcaption{ResNet}
            \label{fig_rmse_0_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/0_100/psnr_0_100.pdf}
            % \subcaption{MAE}
            \label{fig:psnr_0_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/0_100/ssim_0_100.pdf}
            \label{fig:ssim_0_100}
        \end{minipage} \\
        
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/80_100/mae_80_100.pdf}
            % \subcaption{ResNet}
            \subcaption{}
            \label{fig:ma_0_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/80_100/rmse_80_100.pdf}
            % \subcaption{ResNet}
            \subcaption{}
            \label{fig:rmse_80_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/80_100/psnr_80_100.pdf}
            % \subcaption{RMSE}
            \subcaption{}
            \label{fig:psnr_80_100}
        \end{minipage} &
        \begin{minipage}[t]{\myimgwidth\hsize}
            \centering
            \includegraphics[width=\linewidth]{images/score_fig/80_100/ssim_80_100.pdf}
            \subcaption{}
            \label{fig:ssim_80_100}
        \end{minipage} \\
    \end{tabular}
    
    
    \caption{Quality evaluation of frames degraded by JPEG transcoding.
    Top: Compression strength increased by 10 from 0 to 100. Bottom: compressive strength increased by 1 from 80 to 100.
    (a) MAE．
    (b) RMSE．
    (c) PSNR．
    (d) SSIM．}
    \label{fig:jpeg_quality_evaluate}

\end{figure*}


